An Analytical Model for Loc/ID Mappings Caches

Concerns regarding the scalability of the inter-domain routing have encouraged researchers to start elaborating a more robust Internet architecture. While consensus on the exact form of the solution is yet to be found, the need for a semantic decoupling of a node's location and identity is generally accepted as a promising way forward. However, this typically requires the use of caches that store temporal bindings between the two namespaces, to avoid hampering router packet forwarding speeds. In this article, we propose a methodology for an analytical analysis of cache performance that relies on the working-set theory. We first identify the conditions that network traffic must comply with for the theory to be applicable and then develop a model that predicts average cache miss rates relying on easily measurable traffic parameters. We validate the result by emulation, using real packet traces collected at the egress points of a campus and an academic network. To prove its versatility, we extend the model to consider cache polluting user traffic and observe that simple, low intensity attacks drastically reduce performance, whereby manufacturers should either overprovision router memory or implement more complex cache eviction policies.

==> ssec_lisp_background.tex <==
The Locator/ID Separation Protocol (LISP)~\cite{saucez:lisp} is one of the
proposals that implement the loc/id split paradigm and which has recently
undergone IETF standardization~\cite{rfc6830}. It counts with the support of a
sizable community, spanning both academia and industry, and relies on a large
international experimental testbed~\cite{lisp:testbed} (over 32 countries)
that is dedicated to its development. 

One of the definining features of LISP, that also distinguishes it from many
of its competitors, is its support for an incremental deployment. To
facilitate transition from the current Internet infrastructure, both identity
and location namespaces use the existing IP addressing scheme. As a result,
the split does not affect routing within existing stub or transit networks.
Nevertheless, as identifiers and locators bear relevance only within their
respective namespaces, a form of conversion, from one to the other, has to be
performed at border points between core and edge networks. LISP routers make
us of map-and-encap~\cite{rfc1955} to convey both location and identity
information in the same packet. 

\begin{figure}[t]
    \centering
    \includegraphics[width=80mm,keepaspectratio=true]{./figures/lisp-arch.pdf}
    \caption{Example packet exchange between $EID_{SRC}$ and $EID_{DST}$ with
    LISP. Following intra-domain routing, packets reach $xTR_{A}$ which
    obtains a mapping binding $EID_{DST}$ to $RLOC_{B1}$ and $RLOC_{B2}$ from the mapping-system
    (steps 1-3). From the mapping, $xTR_{A}$ chooses $RLOC_{B1}$ as destination
    and then forwards towards it the encapsulated packets over the Internet's
    core (step 4). $xTR_{B}$ decapsulates the packets and forwards them to their
    intended destination. }
    \label{fig:lisp-arch}
\end{figure}

Prior to forwarding a host generated packet, a LISP router maps the
destination address, or Endpoint IDentifier (EID), to a corresponding
destination Routing LOCator (RLOC) by means of a LISP specific mapping
system~\cite{draft:lisp-alt,draft:lisp-ddt,jakab:lisp-tree}. Once a mapping
is obtained, the border router tunnels the packet from source edge to
corresponding destination edge network by means of an encapsulation with a
LISP-UDP-IP header. The outer IP header addresses are the RLOCs pertaining to
the corresponding border routers (see Fig.~\ref{fig:lisp-arch}). At the
receiving router, the packet is decapsulated and forwarded to its intended
destination. In LISP parlance, the source router, that performs the
encapsulation, is called an Ingress Tunnel Router (ITR) whereas the one
performing the decapsulation is named the Egress Tunnel Router (ETR). One that
performs both functions is referred to as an xTR. 

%Being , the packet throughput of an ITR is highly dependent on the time needed
%to obtain a mapping. In consequence, all ITRs are provisioned with a cache,
%called map-cache, that stores the recently used EID-prefix-to-RLOC mappings to
%avoid frequent EID resolutions through the mapping system.

Since LISP implements a loc/id split, ITRs are provisioned with map-caches
that store recently used EID-prefix-to-RLOC mapings. Stale entries are avoided
with the help of timeouts, called \emph{time to live} (TTL), that mappings
carry as attributes. Consistency is ensured through proactive LISP mechanisms
through which the xTR owner of an updated mapping informs its peers of the
change. As previously discussed, the map-cache is most efficient in situations
when destination EIDs present high temporal and/or spatial locality and its
size depends on the diversity of the visited destinations. As a result,
performance depends entirely on map-cache provisioned size, traffic
characteristics and the eviction policy set in place. 

We dedicate the remainder of the paper to finding and evaluating the relation
between parameters like cache size, performance and locality of traffic. 



